Evolving Domain Adaptation of Pretrained Language Models for Text Classification

Adapting pre-trained language models (PLMs) for time-series text classification amidst evolving domain shifts (EDS) is critical for maintaining accuracy in applications like stance detection. This study benchmarks the effectiveness of evolving domain adaptation (EDA) strategies, notably self-training, domain-adversarial training, and domain-adaptive pretraining, with a focus on an incremental self-training method. Our analysis across various datasets reveals that this incremental method excels at adapting PLMs to EDS, outperforming traditional domain adaptation techniques. These findings highlight the importance of continually updating PLMs to ensure their effectiveness in real-world applications, paving the way for future research into PLM robustness against the natural temporal evolution of language.

==> algorithms/dynamic_example_selection.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwIn{Source domain $\Dcal_0$, target domains $\Dcal_{1:T}$, \#examples per class as $k$, label space $\Ycal$}
Initialize buffer $\Bcal_0 = \Dcal_0$, buffer size $b=|\Dcal_0|$\; 
\For{$t = 1$ to $T$}{
    Initialize the in-context example set $\Ccal_{t-1}=\emptyset$\;
    \For{$y$ in $\Ycal$}{
        Compute mean embedding $\ub_{t-1}^y$ by Eq.~(\ref{eq:find_mean_emb_1})\; 
        Find most-representative example $(x_\text{rep}, y)$\; 
        Collect the in-context example $\Ccal_{t-1} = \Ccal_{t-1} \cup \{(x_\text{rep}, y)\}$;         
    }
Create a few-shot prompt using $x'_i=\mathcal{T}(x_i, \Ccal_{t-1})$, $\forall x_i \in \Dcal_t$\; 
Obtain pseudo-label $\tilde{y}_i=v^{-1}(f_\text{LLM}(x'_i)),\forall v^{-1}(x'_i) \in \Dcal_t$\; 

Update $\Bcal_{t}$ by FIFO in Eq.~(\ref{eq:buffer_fifo});
}
\KwOut{$\{C_t\}_{t=0}^{T-1}$, the set of all in-context examples} 
\caption{Online Update of In-context Examples (OIE)}
\label{algo:dynamic_example_selection}
\end{algorithm}

% for every instance $x_i \in \Dcal_{t}$, we then construct the prompt string $x'_i=\mathcal{T}(x_i, \Ccal_{t-1},I)$
% \begin{algorithm}
% \label{algo:dynamic_example_selection}
% \DontPrintSemicolon
% \KwIn{Source domain $\Dcal_0$, target domains $\Dcal_{1:T}$, \#examples per class as $k$, \#class as $M$}
% Initialize buffer $\Bcal_0 = \Dcal_0$, buffer size $b=|\Dcal_0|$\;
% \For{$t = 1$ to $T$}{
%     \For{$y=1$ to $M$}{
%         Compute mean embedding $\mu_{t-1}^y = h(\Bcal_{t-1}, y)$\; 
%         Select in-context examples $\Ccal_{t-1} = \{(x_{rep}^y, v(y_{rep}^y))|y \in \Ycal\}$\;
%     }
%     Create a few-shot prompt using $C_{t-1} = \bigcup_{y=1}^{M} C_{t-1}^y$\;
    
%     Obtain pseudo-label $\tilde{y}_i = f_\text{LLM}(x_i, C_{t-1}), \forall x_i \in \Dcal_{t}$\;
    
%     Update $\Bcal_{t} = \text{FIFO}(\Bcal_{t-1} \cup \{(x_i, \tilde{y}_i)\}_{i=1}^{n_{t}}, b)$ \;
% }
% \KwOut{$\{C_t\}_{t=0}^{T-1}$, the set of all in-context examples over time}
% \caption{Dynamic In-context Example Selection for Online Learning}
% \end{algorithm}


==> figures/correlation_scatter_plot/pubcls_mmd_normlized_score_by_domain_scatter.tex <==
\begin{figure}[tbp!] % use figure for single-column figures
\centering
\includegraphics[width=1.1\linewidth]{figures/correlation_scatter_plot/pubcls_mmd_normlized_score_by_domain_scatter.pdf}
\vspace{-4mm}
\caption{Scatter plot depicting, within the PUBCLS dataset, the correlation between MMD (Maximum Mean Discrepancy) from the source domain $\Dcal_{0}$ to each target domain (X-axis) and the relative gain $\Delta_{\text{norm}}$ (\%) (Y-axis) for each target domain. Each dot represents a target domain, with \textcolor{red}{red} dots denoting results from \onlinecum and \textcolor{teal}{green} dots from \onlinebuf. The linear regression lines for both methods are overlaid, along with the Pearson's $r$ to indicate the strength of the relationship.}
\label{fig:scatter_plot_pubcls}
\vspace{-5mm}
\end{figure}


==> figures/correlation_scatter_plot/scierc_mmd_normlized_score_by_domain_scatter.tex <==
\begin{figure}[tbp!] % use figure for single-column figures
\centering
\includegraphics[width=1.1\linewidth]{figures/correlation_scatter_plot/scierc_mmd_normlized_score_by_domain_scatter.pdf}
\vspace{-4mm}
\caption{Scatter plot depicting, within the SCIERC dataset, the correlation between MMD (Maximum Mean Discrepancy) from the source domain $\Dcal_{0}$ to each target domain (X-axis) and the relative gain $\Delta_{\text{norm}}$ (\%) (Y-axis) for each target domain. Each dot represents a target domain, with \textcolor{red}{red} dots denoting results from \onlinecum and \textcolor{teal}{green} dots from \onlinebuf. The linear regression lines for both methods are overlaid, along with the Pearson's $r$ to indicate the strength of the relationship.}
\label{fig:scatter_plot_scierc}
\vspace{-5mm}
\end{figure}


==> figures/correlation_scatter_plot/wtwt_mmd_normlized_score_by_domain_scatter.tex <==
\begin{figure}[tbp!] % use figure for single-column figures
\centering
\includegraphics[width=1.1\linewidth]{figures/correlation_scatter_plot/wtwt_mmd_normlized_score_by_domain_scatter.pdf}
\vspace{-4mm}
\caption{Scatter plot depicting, within the WTWT dataset, the correlation between MMD (Maximum Mean Discrepancy) from the source domain $\Dcal_{0}$ to each target domain (X-axis) and the relative gain $\Delta_{\text{norm}}$ (\%) (Y-axis) for each target domain. Each dot represents a target domain, with \textcolor{red}{red} dots denoting results from \onlinecum and \textcolor{teal}{green} dots from \onlinebuf. The linear regression lines for both methods are overlaid, along with the Pearson's $r$ to indicate the strength of the relationship.}
\label{fig:scatter_plot_wtwt}
\vspace{-5mm}
\end{figure}


==> figures/domain_divergences.tex <==
\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/domain_divergences/covid_vaccine/wasserstein_infinity_dist/div_P_X_joint_Y.pdf}}
\centerline{\includegraphics[width=\columnwidth]{figures/domain_divergences/covid_vaccine/wasserstein_infinity_dist/div_P_X.pdf}}
\centerline{\includegraphics[width=\columnwidth]{figures/domain_divergences/covid_vaccine/wasserstein_infinity_dist/div_P_Y.pdf}}
\caption{Divergences from the source domain in the COVID Vaccine dataset. The X-axis shows time, while the Y-axis shows Wasserstein-$\infty$ distance, a measure of divergence between two probability distributions. The graphs show the presence of both a Covariate and Label shift over time.}
\label{fig:covid-div-wasserstein-infty}
\end{center}
\vskip -0.3in
\end{figure}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/domain_divergences/covid_vaccine/wasserstein_infinity_dist/div_P_X_given_Y=y.pdf}}
\caption{Divergences from the source domain in the COVID Vaccine dataset. The X-axis shows time, while the Y-axis shows Wasserstein-$\infty$ distance, a measure of divergence between two probability distributions. Each line represents divergence of the conditional distribution $P(X|Y=y)$}
\label{fig:covid-div-wasserstein-infty-conditional}
\end{center}
\vskip -0.3in
\end{figure}

==> figures/domain_divergences/distance_mat/covid_vaccine/cosine_dist/heatmap_marginal_cosine_distance_overlay.tex <==
% \begin{figure}[H]
\begin{figure}[htbp!]
\centering
\includegraphics[width=\linewidth]{figures/domain_divergences/distance_mat/covid_vaccine/cosine_dist/heatmap_marginal_cosine_distance_overlay_fig.pdf}
\caption{TODO}
\label{fig:mat_dist_cosine_covid_not_marginal}
\end{figure}


==> figures/domain_divergences/distance_mat/dataset_merged/cosine_dist/heatmap_marginal_cosine_distance_overlay_merged.tex <==
\begin{figure*}[htbp!] % use figure* for two-column figures
\centering
\begin{subfigure}{0.475\textwidth} % width of left subfigure
\centering
\includegraphics[width=\linewidth]{figures/domain_divergences/distance_mat/covid_vaccine/cosine_dist/heatmap_marginal_cosine_distance_overlay.pdf}
\caption{COVID Dataset} % caption for left subfigure
\label{fig:mat_dist_cosine_covid_not_marginal}
\end{subfigure}
\hfill
\begin{subfigure}{0.475\textwidth} % width of right subfigure
\centering
\includegraphics[width=\linewidth]{figures/domain_divergences/distance_mat/wtwt/cosine_dist/heatmap_marginal_cosine_distance_overlay.pdf}
\caption{WTWT Dataset} % caption for right subfigure
\label{fig:mat_dist_cosine_wtwt_marginal}
\end{subfigure}
\caption{TODO} % caption for the whole figure
\label{fig:merged_figure}
\end{figure*}

==> figures/domain_divergences/distance_mat/dataset_merged/mmd/heatmap_marginal_mmd_overlay_merged.tex <==
\begin{figure*}[htbp!] % use figure* for two-column figures
\centering
\begin{subfigure}{0.48\textwidth} % width of left subfigure
\centering
\includegraphics[width=\linewidth]{figures/domain_divergences/distance_mat/covid_vaccine/mmd/heatmap_marginal_mmd_overlay.pdf}
\caption{COVID Dataset} % caption for left subfigure
\label{fig:mat_dist_cosine_covid_marginal}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\textwidth} % width of right subfigure
\centering
\includegraphics[width=\linewidth]{figures/domain_divergences/distance_mat/wtwt/mmd/heatmap_marginal_mmd_overlay.pdf}
\caption{WTWT Dataset} % caption for right subfigure
\label{fig:mat_dist_cosine_wtwt_marginal}
\end{subfigure}
\caption{Maximum Mean Discrepancy (MMD) matrix for (a) the COVID dataset and (b) the WTWT dataset. Each cell represents the MMD between a pair of domains, calculated based on the marginal distribution of text embeddings $P_{g(\Xcal)}$ projected by the E5-Large-V2 model. The color gradient ranges from white (representing zero discrepancy) to darker shades of red (indicating larger discrepancies). Please note that the numbers in the heatmap are in the units of $10^{-3}$ and $10^{-2}$ for (a) and (b), respectively.} % caption for the whole figure
\label{fig:mat_dist_cosine_marginal_merged}
\end{figure*}

==> figures/prompting_gda/covid_vaccine/prompting_chatgpt_gda_covid.tex <==
\begin{figure}[tbp!] % use figure for single-column figures
\centering
\includegraphics[width=0.9\linewidth]{figures/prompting_gda/covid_vaccine/plot_prompting_gpt_chat_turbo_3_5_covid_f1_macro.pdf}
\vspace{-4mm}
\caption{Prompting using ChatGPT with in-context learning over target domains on the COVID Dataset. The x-axis denotes the domains in order. The Macro-F1 score for each domain is plotted on the y-axis. Three different prompting methods are represented in this plot: \promptzero (\textcolor{darkyellow}{yellow}), \promptsource (\textcolor{blue}{blue}), \onlineexp (\textcolor{teal}{green}).}
\label{fig:prompting_gda_covid}
\vspace{-4mm}
\end{figure}

==> figures/prompting_gda/dataset_merged/merged_prompting_chatgpt_gda.tex <==
\begin{figure*}[htbp!] % use figure* for two-column figures
\centering
\begin{subfigure}{0.48\textwidth} % width of left subfigure
\centering
\includegraphics[width=\linewidth]{figures/prompting_gda/covid_vaccine/plot_prompting_gpt_chat_turbo_3_5_covid_f1_macro.pdf}
\caption{COVID Dataset} % caption for left subfigure
\label{fig:merged_prompting_gda_covid}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\textwidth} % width of right subfigure
\centering
\includegraphics[width=\linewidth]{figures/prompting_gda/wtwt/plot_prompting_gpt_chat_turbo_3_5_wtwt_f1_macro.pdf}
\caption{WTWT Dataset} % caption for right subfigure
\label{fig:merged_prompting_gda_covid}
\end{subfigure}
\caption{Prompting using ChatGPT with in-context learning over time on both the (a) COVID and (b) WTWT dataset. The x-axis denotes the domains, beginning with the source domain and all subsequent target domains. The Macro-F1 score for each domain are plotted on the y-axis. Three different prompting methods are represented in these plots: \promptzero (\textcolor{darkyellow}{yellow}), \promptsource (\textcolor{blue}{blue}), \onlineexp (\textcolor{teal}{green}).} % caption for the whole figure
\label{fig:merged_prompting_gda}
\end{figure*}

==> figures/prompting_gda/dataset_merged/merged_prompting_flan_t5_xxl_gda.tex <==

\begin{figure*}[htbp!] % use figure* for two-column figures
\centering
\begin{subfigure}{0.48\textwidth} % width of left subfigure
\centering
\includegraphics[width=\linewidth]{figures/prompting_gda/covid_vaccine/plot_prompting_flan_t5_xxl_covid_f1_macro.pdf}
\caption{COVID Dataset} % caption for left subfigure
\label{fig:mat_dist_cosine_covid_marginal}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\textwidth} % width of right subfigure
\centering
\includegraphics[width=\linewidth]{figures/prompting_gda/wtwt/plot_prompting_flan_t5_xxl_wtwt_f1_macro.pdf}
\caption{WTWT Dataset} % caption for right subfigure
\label{fig:mat_dist_cosine_wtwt_marginal}
\end{subfigure}
\caption{Prompting with in-context learning over time on both the (a) COVID and (b) WTWT dataset. The x-axis denotes the domains, beginning with the source domain and all subsequent target domains. The Macro-F1 score for each domain are plotted on the y-axis. Three different prompting methods are represented in these plots: \promptzero (\textcolor{darkyellow}{yellow}), \promptsource (\textcolor{blue}{blue}), \onlineexp (\textcolor{teal}{green}).} % caption for the whole figure
\label{fig:mat_dist_cosine_marginal_merged}
\end{figure*}

==> figures/prompting_gda/wtwt/prompting_chatgpt_gda_wtwt.tex <==
\begin{figure}[htbp!] % use figure for single-column figures
\centering
\includegraphics[width=\linewidth]{figures/prompting_gda/wtwt/plot_prompting_gpt_chat_turbo_3_5_wtwt_f1_macro.pdf}
\caption{Prompting using ChatGPT with in-context learning over domains on the WTWT Dataset. The x-axis denotes the domains, beginning with the source domain and all subsequent target domains. The Macro-F1 score for each domain is plotted on the y-axis. Three different prompting methods are represented in this plot: \promptzero (\textcolor{darkyellow}{yellow}), \promptsource (\textcolor{blue}{blue}), \onlineexp (\textcolor{teal}{green}). The actual time stamp of the start of each domain is appended to the domain name in the format of (YY-MM).}
\label{fig:prompting_gda_wtwt}
\end{figure}


==> figures/tuning_gda/covid_vaccine/tuning_gda_covid.tex <==
\begin{figure}[tbp!] % use figure for single-column figures
\centering
\includegraphics[width=0.9\linewidth]{figures/tuning_gda/covid_vaccine/plot_tuning_covid_f1_macro_vc3.pdf}
\vspace{-4mm}
\caption{Fine-tuning with self-training over domains on the COVID dataset. The x-axis denotes the domains. The Macro-F1 score for each domain are plotted on the y-axis. Five different fine-tuning methods are represented in this plot: \tunesource (\textcolor{blue}{blue}), \onlinebuf (\textcolor{teal}{green}), \onlinecum (\textcolor{red}{red}), \offline (\textcolor{violet}{purple}), and \tunetrue (\textcolor{darkgray}{grey}).}% caption for the figure
\label{fig:tuning_gda_covid}
\vspace{-4mm}
\end{figure}


==> figures/tuning_gda/dataset_merged/merged_tuning_wtwt_pubcls_scierc_gda.tex <==
\begin{figure*}[htbp!] 
\centering
\begin{subfigure}{\linewidth} % width of top subfigure
\centering
\includegraphics[width=\linewidth]{figures/tuning_gda/wtwt/plot_tuning_wtwt_f1_macro_vwt2.pdf}
\caption{WTWT Dataset} % caption for top subfigure
\label{fig:merged_tuning_gda_wtwt}
\end{subfigure}
\vspace{1em} % space between subfigures

\begin{subfigure}{\linewidth} % width of middle subfigure
\centering
\includegraphics[width=\linewidth]{figures/tuning_gda/pubcls/plot_tuning_pubcls_f1_macro_pubt2.pdf}
\caption{PUBCLS Dataset} % caption for middle subfigure
\label{fig:merged_tuning_gda_pubcls}
\end{subfigure}
\vspace{1em} % space between subfigures

\begin{subfigure}{\linewidth} % width of bottom subfigure
\centering
\includegraphics[width=\linewidth]{figures/tuning_gda/sci_erc/plot_tuning_scierc_f1_macro_scit2.pdf}
\caption{SCIERC Dataset} % caption for bottom subfigure
\label{fig:merged_tuning_gda_scierc}
\end{subfigure}

\caption{Fine-tuning with self-training over domains on (a) WTWT, (b) PUBCLS, and (c) SCIERC datasets. The x-axis denotes the domains, beginning with the source domain and all subsequent target domains. The Macro-F1 score for each domain are plotted on the y-axis. Five different fine-tuning methods are represented in these plots: \tunesource (\textcolor{blue}{blue}), \onlinebuf (\textcolor{teal}{green}), \onlinecum (\textcolor{red}{red}), \offline (\textcolor{violet}{purple}), and \tunetrue (\textcolor{darkgray}{grey}).} % caption for the whole figure
\label{fig:merged_tuning_gda_wtwt_pubcls_scierc}
\end{figure*}


==> figures/tuning_gda/pubcls/tuning_gda_pubcls.tex <==
\begin{figure}[H] % use figure for single-column figures
\centering
\includegraphics[width=\linewidth]{figures/tuning_gda/pubcls/plot_tuning_pubcls_f1_macro_pubt2.pdf}
\caption{Fine-tuning with self-training over domains on the PUBCLS dataset. The x-axis denotes the domains, beginning with the source domain and all subsequent target domains. The Macro-F1 score for each domain are plotted on the y-axis. Five different fine-tuning methods are represented in this plot: \tunesource (\textcolor{blue}{blue}), \onlinebuf (\textcolor{teal}{green}), \onlinecum (\textcolor{red}{red}), \offline (\textcolor{violet}{purple}), and \tunetrue (\textcolor{darkgray}{grey}).} % caption for the figure
\label{fig:tuning_gda_wtwt}
\end{figure}


==> figures/tuning_gda/sci_erc/tuning_gda_sci_erc.tex <==
\begin{figure}[H] % use figure for single-column figures
\centering
\includegraphics[width=\linewidth]{figures/tuning_gda/sci_erc/plot_tuning_scierc_f1_macro_scit2.pdf}
\caption{Fine-tuning with self-training over domains on the SCIERC dataset. The x-axis denotes the domains, beginning with the source domain and all subsequent target domains. The Macro-F1 score for each domain are plotted on the y-axis. Five different fine-tuning methods are represented in this plot: \tunesource (\textcolor{blue}{blue}), \onlinebuf (\textcolor{teal}{green}), \onlinecum (\textcolor{red}{red}), \offline (\textcolor{violet}{purple}), and \tunetrue (\textcolor{darkgray}{grey}).} % caption for the figure
\label{fig:tuning_gda_wtwt}
\end{figure}


==> figures/tuning_gda/wtwt/tuning_gda_wtwt.tex <==
\begin{figure}[H] % use figure for single-column figures
\centering
\includegraphics[width=\linewidth]{figures/tuning_gda/wtwt/plot_tuning_wtwt_f1_macro_vwt2.pdf}
\caption{Fine-tuning with self-training over domains on the WTWT dataset. The x-axis denotes the domains, beginning with the source domain and all subsequent target domains. The Macro-F1 score for each domain are plotted on the y-axis. Five different fine-tuning methods are represented in this plot: \tunesource (\textcolor{blue}{blue}), \onlinebuf (\textcolor{teal}{green}), \onlinecum (\textcolor{red}{red}), \offline (\textcolor{violet}{purple}), and \tunetrue (\textcolor{darkgray}{grey}).} % caption for the figure
\label{fig:tuning_gda_wtwt}
\end{figure}


==> rebuttal/sections/review_1.tex <==
\section{Review 1}
\label{sec:review-1}
Official Review of Submission1109 by Reviewer 24y4

\subsection*{Paper Topic And Main Contributions:}
The paper addresses the challenge of performance degradation in pre-trained language models due to natural evolving domain shifts in dynamic real-world environments. It introduces two adaptation strategies to mitigate this issue: self-training with pseudo-labeling for small language models (SLMs) and a tuning-free, in-context learning approach for large language models (LLMs). The proposed methods are validated through extensive experiments on longitudinal social media datasets. Additionally, the paper contributes a novel COVID-19 vaccination stance detection dataset, which serves as a benchmark for evaluating pre-trained language models within evolving domain adaptation settings.

\subsection*{Reasons To Accept:}

1. This paper addresses an important and timely issue of performance degradation in pre-trained language models due to evolving domain shifts. This challenge is highly relevant in today's dynamic real-world environments.

2. The introduction of two adaptation strategies catering to both small and large language models demonstrates a comprehensive approach to tackling the domain shift problem. These strategies cater to different scales of models, enhancing the paper's practical relevance.

3. This paper supports its proposed strategies with extensive experiments on real-world social media datasets. This empirical validation strengthens the significance and impact of the contributions.

\subsection*{Reasons To Reject:}

1. While the paper mentions the superiority of the proposed methods over unadapted baselines, it should include a more detailed comparative analysis. How do the proposed strategies compare to existing domain adaptation methods in terms of performance, efficiency, and ease of implementation?

2.The experiments are conducted on social media datasets, which might raise questions about the generalizability of the proposed methods to other text domains. A discussion on the potential applicability of the methods in diverse domains would strengthen the paper's claims.

\subsection*{Questions For The Authors:}

In the context of the COVID-19 vaccination stance detection dataset, how do you ensure the quality and reliability of the annotations, given the sensitivity of the topic? Are there potential biases that could impact the benchmark's effectiveness?

\subsection*{Ratings}

Soundness: 3: Good: This study provides sufficient support for its major claims/arguments, some minor points may need extra support or details.

Excitement: 3: Ambivalent: It has merits (e.g., it reports state-of-the-art results, the idea is nice), but there are key weaknesses (e.g., it describes incremental work), and it can significantly benefit from another round of revision. However, I won't object to accepting it if my co-reviewers champion it.

Reproducibility: 4: Could mostly reproduce the results, but there may be some variation because of sample variance or minor variations in their interpretation of the protocol or method.

Ethical Concerns: No

Reviewer Confidence: 4: Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.

\section*{\sn{Response to Review 1}}

\paragraph{Q1.} \textit{"A more detailed comparative analysis: How do the proposed strategies compare to existing domain adaptation methods in terms of performance, efficiency, and ease of implementation?"}

Thank you for the suggestion. We conducted additional experiments to compare our strategies with two additional domain adaptation methods: DANN (suggested by Reviewer 1rUf) [1,2] and continued pre-training (i.e., DAPT suggested by Reviewers 1rUf and iqaY) [3,4]. Table 1 shows the additional results.

% A common adaptation method is Domain Adversarial Neural Networks (DANN), as pointed out by reviewer 1rUf as well. We examined it in our early experiments but did not include the results due to page limit. 

\input{rebuttal/tables/other_adapted_methods}

- Following the DANN literature [1,2], for each source-target domain pair, we employ DANN by training a pretrained BERT model (same backbone as the other methods in our paper) on (i) an adversarial loss to learn domain-invariant features and (ii) a downstream classification loss with equal weights, i.e., total loss = cross-entropy loss + adversarial loss. From the results, we find that DANN surpasses the baseline Src-only while underperforming OBS. Notably, we also observe that DANN's performance drops as the time step of target domains increases, possibly due to growing divergence between source domain $\Dcal_0$ and target domain $\Dcal_{t}$ (see Figure 4 and 7 in the main paper).%, complicating the learning of domain-invariant features.%The trained DANN is then evaluated on each target domains at each time step.


% The DANN comprises three components: the feature extractor, label predictor, and domain classifier. In our study, for the feature extractor, we utilize the same pretrained BERT model as in the main paper. Its output, denoted as $f$, branches into two paths. One leads to the label predictor, calculating a cross-entropy loss ($loss_{CE}$). The other feeds the domain classifier, resulting in a domain adversarial loss ($loss_{ADV}$). With the domain adversarial loss, DANN encourages the extractor to learn domain-invariant features. Thus, after training, DANN should generalize to the target domain. The total minimized loss is $loss = loss_{CE} + w_{adv} \times loss_{ADV}$, where $w_{adv}$ is the weight of the adversarial loss (set to 1). Since there are $T$ target domains for each dataset, we train $T$ separate DANN models.

% We use the Python Transfer Learning Library to build our implementation of the DANN.

% DANN's performance is benchmarked against our methods (OBS, OCS, OS) shown in the table below. Although DANN surpasses the baseline Src-only, it falls short of OBS. Notably, we also observe that DANN's performance drops as $t$ rises, possibly due to growing divergence between source domain $\Dcal_0$ and target domain $\Dcal_{t}$ (as shown in Figure 4 and 7), complicating the learning of domain-invariant features.

- We adopt the domain-adaptive pretraining (DAPT) method [3,4] in the EDA setting. Specifically, we first continue pre-training the BERT model on each target-domain data, and then fine-tuning the model further on source-domain classification. We use the same hyperparamters as [3] for DAPT. Similarly, we find that DAPT outperforms Src-only while still lagging behind OBS. Note that, [3] found that the gain from DAPT is limited given target labeled data. Consistent with their finding, OBS does leverage target pseudo-labeled data for fine-tuning, thus reaching a better overall performance.


% Aside from DANN, as suggested by reviewer 1rUf and reviewer iqaY, we also consider \textit{continued pre-training} as another adaptation method [3,4]. In [3], the authors show that, by using domain-adaptive pretraining (DAPT) to continue pretraining an GPT-2 model on a time-specific domain, combined with time-specific fine-tuning (fine-tuning with the labeled data from the time step of interest), the model reaches a higher performance compared to a generic pretrained GPT-2. Following [3], for each unlabeled target domain, we adopt DAPT to further pretrain the BERT model. Note that, unlike [3], we assume the evolving domain adaptation (EDA) setting, where there is no labels available in the target domains. Therefore, after DAPT, we further fine-tune the BERT model with the labels from the source domain. We use the same hyperparamters as [3] for DAPT.

% The table above shows that DAPT does improve upon the Src-only baseline. However, the model performance is still worse than OBS. This is consistent with [3], where they found that the gain of using DAPT is smaller than using time-specific fine-tuning. Note that, in contrast to DAPT, OBS does leverage time-specific fine-tuning, albeit with pseudolabels, and therefore reaches a better overall performance.

\paragraph{Q2.} \textit{"Generalizability to other text domains and a discussion on the potential applicability of the methods in diverse domains"}

Thank you for the suggestion. We expand the datasets to include texts from domains other than social media. Specifically, we add a dataset of scientific articles (SCIERC) [5], and another of news articles (PUBCLS) [6]. SCIERC consists of about 8K scientific entities in the abstract of computer science papers published from 1980 to 2016. Each entity is classified into one of the six following categories: task, method, metric, material, other-six scientific-term, or generic. We use the same time partitions in [3] to split articles by time. We use 1980-1999 as the labeled source domain, and 2000-2004, 2005-2009, 2010-2016 as the three following unlabeled target domains. PUBCLS contains 67k documents published by different publishers from 2009 to 2016. The task is to classify documents into its publisher. We use the same partition as in [3], and define 2009-2010 as the source domain and the rest as the target domains.

The results below echo the discoveries in our main paper, where OS>OCS>OBS>Src-only for fine-tuning, and OIE>Src-only for prompting. Therefore, we believe that the findings from our paper are generalizable and not limited to only the social media domain. %the generalizability of our proposed methods are not limited to social media datasets.

\input{rebuttal/tables/obs_other_datasets}

\input{rebuttal/tables/oie_other_datasets}


\paragraph{Q3.} \textit{"Quality and reliability of the annotations of COVID-19 vaccination stance detection? Are there potential biases?"}

To mitigate potential bias among annotators, all the annotators have to undergo at least 1 month of annotation training sessions. During the training sessions, annotators and experts in the COVID-19 vaccination narrative have weekly meetings to have deliberative discussions on ambiguous cases. Annotators are requested to focus only on the literal textual content according to a codebook, rather than politicized cues. The codebook is developed based on prior literature about COVID-19 vaccine narratives [7,8].

In addition, to ensure the reliability of human annotation, we train the eight annotators to make sure their inter-rater reliability is high enough (Appendix C.4). Furthermore, we randomly select 300 tweets and have an expert in the COVID-19 vaccination narrative to annotate them (Appendix C.4).  The agreement rate between the majority vote of these X raters and the expert is 89.7\% (Table 7).

\subsection*{References}

[1] Ganin, Y., Ustinova, E., Ajakan, H., Germain, P., Larochelle, H., Laviolette, F., ... \& Lempitsky, V. (2016). Domain-adversarial training of neural networks. The journal of machine learning research, 17(1), 2096-2030.

[2] Tzeng, E., Hoffman, J., Saenko, K., \& Darrell, T. (2017). Adversarial discriminative domain adaptation. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 7167-7176).

[3] Luu, K., Khashabi, D., Gururangan, S., Mandyam, K., \& Smith, N. A. (2022, July). Time Waits for No One! Analysis and Challenges of Temporal Misalignment. In Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (pp. 5944-5958).

[4] Gururangan, S., Marasović, A., Swayamdipta, S., Lo, K., Beltagy, I., Downey, D., \& Smith, N. A. (2020, July). Don’t Stop Pretraining: Adapt Language Models to Domains and Tasks. In Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics (pp. 8342-8360).

[5] Grusky, M., Naaman, M., \& Artzi, Y. (2018). Newsroom: A dataset of 1.3 million summaries with diverse extractive strategies. arXiv preprint arXiv:1804.11283.

[6] Card, D., Boydstun, A., Gross, J. H., Resnik, P., \& Smith, N. A. (2015, July). The media frames corpus: Annotations of frames across issues. In Proceedings of the 53rd Annual Meeting of the Association for Computational Linguistics and the 7th International Joint Conference on Natural Language Processing (Volume 2: Short Papers) (pp. 438-444).

[7] Jiang, X., Su, M. H., Hwang, J., Lian, R., Brauer, M., Kim, S., \& Shah, D. (2021). Polarization over vaccination: Ideological differences in Twitter expression about COVID-19 vaccine favorability and specific hesitancy concerns. Social Media+ Society, 7(3), 20563051211048413.

[8] Lindelöf, G., Aledavood, T., \& Keller, B. (2023). Dynamics of the Negative Discourse Toward COVID-19 Vaccines: Topic Modeling Study and an Annotated Data Set of Twitter Posts. Journal of Medical Internet Research, 25, e41319.






==> rebuttal/sections/review_2.tex <==
\newpage
\section{Review 2}
\label{sec:review-2}
Official Review of Submission1109 by Reviewer 1rUf

\subsection*{Paper Topic And Main Contributions:}
This paper explores evolving domain adaptation by training on pre-trained language models. Two methods are proposed for updating small language models (SLM) and large language models (LLM) respectively. The method for SLM is continuously pseudo-labeling new data from the evolving environment for BERT fine-tuning. The method for LLM is to train the model on additional contexts produced by ChatGPT. Experiments are conducted on two datasets including one provided by this paper and another public one.

\subsection*{Reasons To Accept:}

The story is well written. The experiments and analysis are abundant. The evolving domain adaptation is a meaningful research question for evolving environments.

\subsection*{Reasons To Reject:}

\paragraph{1.} The technical contribution of this paper is incremental and hard to benefit future studies.

The first method proposed by this paper is to continuously fine-tune BERT on the pseudo labels. Nevertheless, pseudo-labeling has been proposed for many years for domain adaptation. It is a basic baseline in unsupervised domain adaptation baseline [1]. The weakness of pseudo-labeling has also been discussed by previous work [2], which shows that pseudo-labeling brings great randomness, especially for those difficult tasks with low prediction accuracy, pseudo labels produced by that kind of model action as noisiness instead of information. Therefore, the proposed method heavily relying on pseudo labels has limited robustness and generalizability to other applications. Additionally, the in-context learning for LLM training is not innovative, the ChatGPT and FLAN-T5 only serve as additional future context, whose performance is therefore limited (see weakness 2).

\paragraph{2.} The performance enhancement is very limited on two datasets.

Referring to Table 2 in this paper, the performance enhancement of in-context learning by FLAN-T5 on new data only goes from 0.784 to 0.788, and 0.562 to 0.563. The experimental results can not convince me that the model works well, especially since the comparison baselines are weak.

\paragraph{3.} The comparison baselines are weak.

There have been a lot of previous studies focusing on training large language models like the reference [3], which conduct continued pretraining on BERT on new data to keep pace with the evolving domain. This paper does not make a comparison with the baseline. There are also some domain adaptation baselines like DANN [4] and other work [5], this paper also misses the comparison.


\subsection*{Missing References:}

[1]Neural Unsupervised Domain Adaptation in NLP—A Survey

[2]Deep Unsupervised Domain Adaptation: A Review of Recent Advances and Perspectives

[3]Time Waits for No One! Analysis and Challenges of Temporal Misalignment

[4]Domain-Adversarial Training of Neural Networks

[5]Contrastive Domain Adaptation for Early Misinformation Detection: A Case Study on COVID-19


\subsection*{Ratings}

Soundness: 2: Borderline: Some of the main claims/arguments are not sufficiently supported, there are major technical/methodological problems

Excitement: 2: Mediocre: This paper makes marginal contributions (vs non-contemporaneous work), so I would rather not see it in the conference.

Reproducibility: 3: Could reproduce the results with some difficulty. The settings of parameters are underspecified or subjectively determined; the training/evaluation data are not widely available.

Ethical Concerns: No

Reviewer Confidence: 4: Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.

\section*{\sn{Response to Review 2}}

We thank the reviewer for the time and helpful comments. We will include the additional results in the next version to strengthen our paper. 

\paragraph{Q1.} \textit{"pseudo-labeling brings great randomness, ..., the proposed method heavily relying on pseudo labels has limited robustness and generalizability to other applications."}

We agree with the reviewer that pseudo-labeling is not new and may suffer from noise. However, we'd like to highlight that our paper mainly focuses on benchmarking pre-trained language models in the EDA setting, which is still missing in the literature. We aim to provide a comprehensive investigation of fine-tuning and prompting strategies in this work, where pseudo-labeling is used as our main fine-tuning strategy in comparison.

To further test the generalizability of our proposed methods in the presence of labeling errors, we additionally include two more challenging datasets from different areas: SCIERC [5] and PUBCLS [6]. We would like to kindly refer you to our response to Reviewer 24y4's Q2. Note that the overall $F_{avg}$ of the baseline model Src-Only score is low for both datasets, indeed posing a challenge to the accuracy of pseudolabeling. %The results below echo the discoveries in our main paper, where OS>OCS>OBS>Src-only for fine-tuning, and OIE>Src-only for prompting. Therefore, we believe that our proposed methods works for more challenging datasets as well, even when the base model performance is low. \jh{Should we add this sentence or paragraph? I don't see a clear connection to the question.}

% It's true that pseudo-labeling itself is an old technique and suffers from inaccuracies. We would like to refer 

\sn{TODO: Aside from DANN, should also include other adaptation baslines.}

% To further test the generalizability of our proposed methods in the presence of labeling errors, we additionally include two more challenging datasets from different areas. We add a dataset of scientific articles - SCIERC [5], and another of news article - PUBCLS [6]. SCIERC consists about 8K of "mentions"(scientific entities) in computer science paper abstracts ranging from 1980 to 2016. Each mention is classified into one of the six following categories, task, method, metric, material, other-six scientific-term, or generic. To partition articles by time, we use the same time partitions in [3]. We use 1980-1999 as the labeled source domain, and 2000-2004, 2005-2009, 2010-2016 as the three following unlabeled target domains. For PUBCLS, it contains 67k of documents published by different publishers from the year of 2009 to 2016. The task is to classify documents into its publisher.  We use the same partition as in [3], and define 2009-2010 as the source domain and the rest as the target domains. Note that the overall $F_{avg}$ of the baseline model Src-Only score is low for both datasets, posing a challenge to the accuracy of pseudolabeling.

% The results below echo the discoveries in our main paper, where OS>OCS>OBS>Src-only for fine-tuning, and OIE>Src-only for prompting. Therefore, we believe that our proposed methods works for more challenging datasets as well, even when the base model performance is low.

\input{rebuttal/tables/obs_other_datasets}

\input{rebuttal/tables/oie_other_datasets}

\paragraph{Q2.} \textit{"The performance enhancement is very limited on two datasets. The experimental results can not convince me that the model works well, especially since the comparison baselines are weak."}

Thank you for pointing out this concern. We investigate the effectiveness of the methods on two additional datasets. Please see the response to Q2 from Reviewer 24y4 for the results on the additional datasets. 

Notably, we also investigate the effectiveness of our online update of in-Context examples (OIE) method using more LLM backbones of different sizes, including FLAN-T5-XL (3B), FLAN-UL2 (20B), text-babbage-001 (3B), text-curie-001 (13B), text-davinci-003 (175B). As shown in the table, OIE outperforms the unadapted Src-Only baseline across all LLMs (except FLAN-XL), which strengthens the findings from our initial submission. In addition, we also observe a scaling effect that all methods could benefit from larger LLMs, thus there may not be a large gap across different methods using smaller LLMs (e.g., FLAN-T5-XXL as used in the submission). %This partially explains a rather small gain of OIE over Src-Only using a large model (FLAN-T5-XXL) in the main paper.

% To further test how robust our proposed online update of in-context examples (OIE) method is, we expand the scope of LLMs to include more models of different sizes - FLAN-T5-XL (3B), FLAN-UL2 (20B), text-babbage-001 (3B), text-curie-001 (13B), text-davinci-003 (175B).

\input{rebuttal/tables/more_llms} %\jh{You may merge this table with the fine-tuned table. }

% As shown in the table above, OIE outperforms the unadapted Src-Only baseline across all LLMs (except FLAN-XL). In addition, we also observe the scaling effect, where the benefit of OIE is more evident for larger LLMs. This could explain why the benefit of OIE on FLAN-T5-XXL in the main paper is rather small.

In addition, we also conduct a statistical test with paired bootstrap resampling [1] and verify the significance of gains from OIE over Src-Only. Specifically, for each target domain, we randomly sample the test set with replacement 1,000 times for testing and derive the 95\% confidence interval of the difference between OIE and the upadapted source-only baseline (Src-Only).  %That is, for each bootstrapped sample, we compute the difference score $\Delta F_\text{avg} = (F_\text{avg} \text{of OIE}) - (F_\text{avg} \text{of Src-Only})$. 

\input{rebuttal/tables/oie_bootstrap}

As shown in the table above, the 95\% confidence interval indicates that, for ChatGPT, text-davinci-003, text-curie-001, and FLAN-T5-UL2, OIE significantly outperforms the Src-Only baseline across both datasets, while OIE shows a significant improvement for FLAN-T5-XXL in COVID but not in WTWT. For smaller LLMs (text-curie-001, FLAN-T5-XL), OIE does not show a significant improvement upon Src-Only. In sum, we find that the merit of OIE hinges on the size of LLM.

Finally, we underscore that OIE is designed specifically for a tuning-free environment. For LLMs, both pre-training and fine-tuning are either prohibitively expensive or unfeasible (as with closed-source models). As a result, we limit our comparisons of OIE to only tuning-free methods (like Src-Only).

\paragraph{3.} \textit{"The comparison baselines are weak. "}

Thanks for the helpful suggestion. We provide additional results on two more baseline methods: DANN and DAPT. We would like to kindly refer you to our response to Q1 from Reviewer 24y4. In short, while DANN and DAPT outperforms the Src-Only baseline, they still underperform OBS.


% Thank you for giving us the opportunity to include more adaptation baselines. A common adaptation method is Domain Adversarial Neural Networks (DANN). We have run it in our early experiments but did not include the results due to page limit. 

% Following the DANN literature [1,2], for each source domain and target domain pair, we train a DANN that utilizes adversarial loss to learn domain-invariant features. The trained DANN is then evaluated on each target domains at each time step.

% The DANN comprises three components: the feature extractor, label predictor, and domain classifier. In our study, for the feature extractor, we utilize the same pretrained BERT model as in the main paper. Its output, denoted as $f$, branches into two paths. One leads to the label predictor, calculating a cross-entropy loss ($loss_{CE}$). The other feeds the domain classifier, resulting in a domain adversarial loss ($loss_{ADV}$). With the domain adversarial loss, DANN encourages the extractor to learn domain-invariant features. Thus, after training, DANN should generalize to the target domain. The total minimized loss is $loss = loss_{CE} + w_{adv} \times loss_{ADV}$, where $w_{adv}$ is the weight of the adversarial loss (set to 1). Since there are $T$ target domains for each dataset, we train $T$ separate DANN models.

% % We use the Python Transfer Learning Library to build our implementation of the DANN.

% DANN's performance is benchmarked against our methods (OBS, OCS, OS) shown in the table below. Although DANN surpasses the baseline Src-only, it falls short of OBS. Notably, we also observe that DANN's performance drops as $t$ rises, possibly due to growing divergence between source domain $\Dcal_0$ and target domain $\Dcal_{t}$ (as shown in Figure 4 and 7), complicating the learning of domain-invariant features.

% \input{rebuttal/tables/other_adapted_methods}

% Aside from DANN, thanks to your suggestion, we also consider \textit{continued pre-training} as another adaptation method [4,5]. In [4], the authors show that, by using domain-adaptive pretraining (DAPT) to continue pretraining an GPT-2 model on a time-specific domain, combined with time-specific fine-tuning (fine-tuning with the labeled data from the time step of interest), the model reaches a higher performance compared to a generic pretrained GPT-2. Following [5], for each unlabeled target domain, we adopt DAPT to further pretrain the BERT model. Note that, unlike [5], we assume the evolving domain adaptation (EDA) setting, where there is no labels available in the target domains. Therefore, after DAPT, we further fine-tune the BERT model with the labels from the source domain. We use the same hyperparamters as [5] for DAPT.

% The table above shows that DAPT does improve upon the Src-only baseline. However, the model performance is still worse than OBS. This is consistent with [5], where they found that the gain of using DAPT is smaller than using time-specific fine-tuning. Note that, in contrast to DAPT, OBS does leverage time-specific fine-tuning, albeit with pseudolabels, and therefore reaches a better overall performance.

\subsection*{References}

[1] Koehn, P. (2004, July). Statistical significance tests for machine translation evaluation. In Proceedings of the 2004 conference on empirical methods in natural language processing (pp. 388-395).

[2] Ganin, Y., Ustinova, E., Ajakan, H., Germain, P., Larochelle, H., Laviolette, F., ... \& Lempitsky, V. (2016). Domain-adversarial training of neural networks. The journal of machine learning research, 17(1), 2096-2030.

[3] Tzeng, E., Hoffman, J., Saenko, K., \& Darrell, T. (2017). Adversarial discriminative domain adaptation. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 7167-7176).

[5] Gururangan, S., Marasović, A., Swayamdipta, S., Lo, K., Beltagy, I., Downey, D., \& Smith, N. A. (2020, July). Don’t Stop Pretraining: Adapt Language Models to Domains and Tasks. In Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics (pp. 8342-8360).

[5] Luu, K., Khashabi, D., Gururangan, S., Mandyam, K., \& Smith, N. A. (2022, July). Time Waits for No One! Analysis and Challenges of Temporal Misalignment. In Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (pp. 5944-5958).


==> rebuttal/sections/review_3.tex <==
\newpage
\section{Review 3}
\label{sec:review-3}
Official Review of Submission1109 by Reviewer 4Jm5

\subsection*{Paper Topic And Main Contributions:}

This paper aims at evolving domain adaptation for text stance classification, such as COVID-related tweet analysis. It introduces a buffer-based self-training approach, which is to control the incorporation of new pseudo-labeled data during fine-tuning ( for BERT ) and in-context prompt learning ( for LLMs like FLAN-T5 and ChatGPT 3.5 API ). The experiments conducted on two datasets, including one proposed by the paper, demonstrate the efficacy of this approach.

Main contribution:
This paper presents a superior self-training approach compared to not employing this method for EDA in text classification.
This paper constructe a new valuable dataset, a random sample of all the English tweets rel- evant to the COVID-19 vaccine, spanning over a period of 19 months (12/2020-06/2022).


\subsection*{Reasons To Accept:}

The evolving domain adaptation task is interesting and meaningful.
The approach's versatility allows it to be applied to both fine-tuning LM and prompting LLMs, enhancing its applicability.

\subsection*{Reasons To Reject:}

\paragraph{1.} The simplicity of the FIFO mechanism in OBS raises concerns about potentially omitting more representative data while adding less informative data. A filter mechanism, akin to OIE, could be beneficial in prioritizing the retention of important data and avoiding catastrophic forgetting. The analysis of OBS/OCS/OS appears to lack depth and brevity, necessitating a more comprehensive examination of the results to strengthen the paper's findings. Also, if OS (no buffer) performs the best, I don't see why it's needed to design methods with dynamic buffer.

\paragraph{2.} The dynamic buffer for fine-tuning models is not truly dynamic in terms of modifying the model architecture. Instead, it pertains to different settings or configurations used outside the model. Just like another hyper-parameter.

\paragraph{3.} In line 419, it is mentioned that "Secondly, OIE significantly outperforms use of static in-context examples from the source domain." However, according to the data presented in Table 2, OIE only exhibits a slight improvement over the src-only approach, especially for FLAN-T5 (0.784 to 0.788) and, (0.562 to 0.563). It is not evident why this marginal difference would be labeled as "significantly" outperforming the src-only method.

\paragraph{4.} In the experiments, no other papers' stance detection methods were used for comparison, apart from the backbones.

\subsection*{Questions For The Authors:}

\paragraph{1.} Is the newly constructed data going to be open-source?

\paragraph{2.} Regarding the buffer used in the study, how was the fixed window size determined?

\paragraph{3.} Considering the potential benefits of adaptability, would a dynamic window size be more effective in the context of your research?



\subsection*{Ratings}

Soundness: 3: Good: This study provides sufficient support for its major claims/arguments, some minor points may need extra support or details.

Excitement: 3: Ambivalent: It has merits (e.g., it reports state-of-the-art results, the idea is nice), but there are key weaknesses (e.g., it describes incremental work), and it can significantly benefit from another round of revision. However, I won't object to accepting it if my co-reviewers champion it.

Reproducibility: 4: Could mostly reproduce the results, but there may be some variation because of sample variance or minor variations in their interpretation of the protocol or method.

Ethical Concerns: No

Reviewer Confidence: 4: Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.

\section*{\sn{Response to Review 3}}

We thank the reviewer for the time and insightful feedback. We will add the additional experiments to update the paper.

\paragraph{Q1.} \textit{"The simplicity of the FIFO mechanism in OBS raises concerns about potentially omitting more representative data while adding less informative data. A filter mechanism, akin to OIE, could be beneficial in prioritizing the retention of important data and avoiding catastrophic forgetting."}

Thank you for your questions. Yes, the fact that OCS outperforms OBS indicates that historical data is indeed important (Table 1, Figure 2). Nonetheless, we would like to highlight that the key property of evolving domain adaptation is that the domain shift happens gradually over time. This assumption is supported by the analysis shown in Figure 4 and 7. Therefore, even though using FIFO mechanism assumes the risk of discarding important data, the newer data that is added to the buffer on average would be more relevant to the query than older data. This is supported by the fact that OBS outperforms the source-only mode.

In addition, we would like to emphasize that the key motivation of OBS is to accommodate the scenario where there is a limited budget in terms of storage and training time. Therefore, OBS operates with a fixed-size buffer where the model is trained (Equation 1), as opposed to OCS which assumes unlimited resources in storing the training data and training time (Equation 2). Note that the training time grows linearly with the training set size.

\paragraph{Q2. } \textit{"The analysis of OBS/OCS/OS appears to lack depth and brevity, necessitating a more comprehensive examination of the results to strengthen the paper's findings."}

Regarding the results of OBS/OCS/OS, we would like to refer you to our additional analysis in our response to Reviewer iqaY670's Q6. We show that the efficacy of buffer-based methods depends on the degree of the domain shift between the source domain and the target domain. The larger the shift, the better our methods perform. We would also like to refer to Table 4 in our paper, where we highlight the factor of pseudolabeling accuracy.

\paragraph{Q3.} \textit{If OS (no buffer) performs the best, I don't see why it's needed to design methods with dynamic buffer.}

Thank you for the question. We would like to emphasize that we consider two different settings---online setting and offline setting (Line 132-144). In the offline setting where all data is available at any time point, you are right that a dynamic buffer may not be necessary since OS performs the best. However, in the online setting, because we only have access to historical data without future data at a given time point, OS is not a viable option.  As a result, only OBS, OCS are possible in the online setting, where we show that both OBS and OCS perform better than the unadapted baseline Src-Only.


\paragraph{Q4.} \textit{"The dynamic buffer for fine-tuning models is not truly dynamic in terms of modifying the model architecture. Instead, it pertains to different settings or configurations used outside the model. Just like another hyper-parameter. Regarding the buffer used in the study, how was the fixed window size determined?"}

When fine-tuning models, for online buffered self-training (OBS), the buffer is "dynamic" in the sense that the training data is updated at each time step  (Algorithm 1). Indeed, OBS does not modify the model architecture. We agree with the reviewer that the size of the fixed window is a hyperparameter. However, we would clarify that we use natural time units (e.g., months) as the fixed window size of the time span, rather than using a fixed number of data points. For OBS and OCS, we use a natural time unit for the fixed time span, i.e., 1 month for COVID and 2 months for WTWT (Line 899-912). Note that the window size determines how often the model is updated. The smaller the window size, the more frequent the update. The reasons are two-fold. Firstly, studies have shown that topics that underlie the discourse on social media show a constant temporal shift over time [1]. Secondly, from a practical point of view, it is easier to maintain a fixed time schedule to update a model rather than relying on a time-varying schedule.

To test the sensitivity to varying window sizes, we test the different sizes of time windows, i.e., 1, 2, 3 months. The detailed result is as follows.

\input{rebuttal/tables/varying_window_size}

The overall trend of results remains the same. Critically, in terms of model performance, OCS > OBS > Src-Only. Notably, the superiority of OCS and OBS compared to Src-Only reduces as the window size increases presumably because the model updates less frequently in the presence of domain shift. Nonetheless, the adaptive methods (OCS and OBS) are always better than the unadapted baseline Src-Only. Therefore, we believe that the benefit of our proposed OCS and OBS is robust against varying window size. 

\paragraph{Q5.} \textit{"In line 419, it is mentioned that "Secondly, OIE significantly outperforms use of static in-context examples from the source domain." However, according to the data presented in Table 2, OIE only exhibits a slight improvement over the src-only approach, especially for FLAN-T5 (0.784 to 0.788) and, (0.562 to 0.563). It is not evident why this marginal difference would be labeled as "significantly" outperforming the src-only method."}

Thanks for raising the concerns. We would like to kindly refer you to our response to Reviewer lrUf's Q2. We expand the scope of LLMs and also conduct statistical significance test, and show that the benefit of OIE holds true for larger LLMs.
% To test how robust our proposed online update of in-context examples (OIE) method is, we expand the scope of LLMs to include more models of different sizes - FLAN-T5-XL (3B), FLAN-UL2 (20B), text-babbage-001 (3B), text-curie-001 (13B), text-davinci-003 (175B). 

% \input{rebuttal/tables/more_llms}

% As shown in the table above, OIE outperforms the unadapted Src-Only baseline across all LLMs (except FLAN-XL). In addition, we also observe the scaling effect, where the benefit of OIE is more evident for larger LLMs. This could explain why the benefit of OIE on FLAN-T5-XXL in the main paper is rather small.

% In addition, we also conduct statistical test with paired bootstrap resampling [2]. For each target domain, we resample from the test set 1000 times, and derive the 95\% confidence interval of the difference between OIE and the upadapted source-only baseline (Src-Only). That is, for each bootstrapped sample, we compute the difference score $\Delta F_\text{avg} = (F_\text{avg} \text{of OIE}) - (F_\text{avg} \text{of Src-Only})$. 



% \input{rebuttal/tables/oie_bootstrap}

% As shown in the table above, the 95\% confidence interval indicates that, for ChatGPT, text-davinci-003, text-curie-001, and FLAN-T5-UL2, OIE significantly outperforms the Src-Only baseline across both datasets, while OIE shows a significant improvement for FLAN-T5-XXL in COVID but not in WTWT. For smaller LLMs (text-curie-001, FLAN-T5-XL), OIE does not show a significant improvement upon Src-Only. In sum, we find that the merit of OIE hinges on the size of LLM.

\paragraph{Q6.} \textit{"In the experiments, no other papers' stance detection methods were used for comparison, apart from the backbones."}

Thank you for giving us the chance to clarify. We design our proposed methods with an attempt to generalize to various text classification tasks, not limiting to stance detection. To demonstrate the generalizability, we investigate the effectiveness of the methods on two additional classification tasks. Please see the response to Q2 from Reviewer 24y4 for the results on the additional datasets. In short, the results echo the discoveries in our main paper, where OS>OCS>OBS>Src-only for fine-tuning, and OIE>Src-only for prompting. 


\paragraph{Q7.} \textit{"Is the newly constructed data going to be open-source?"}

Yes, we plan to release the newly constructed data. To comply with our terms with X (formerly Twitter), we plan to release the tweet IDs, where users can retrieve the text with API. As X’s data-sharing policies are shifting, we will review the updated policies before releasing the tweet IDs publicly. The released data will be limited to non-commercial use cases.

\paragraph{Q8.}\textit{Considering the potential benefits of adaptability, would a dynamic window size be more effective in the context of your research?}

Given that the benefit of our proposed methods is robust against varying window sizes (see our response to your question 4), we believe we have shown that, even with a fixed window size, OBS still outperforms Src-Only. Having a dynamic window size could be an interesting future direction to explore.


\subsection*{References}

[1] Wicke, P., \& Bolognesi, M. M. (2021). Covid-19 discourse on twitter: How the topics, sentiments, subjectivity, and figurative frames changed over time. Frontiers in Communication, 6, 651997.

[2] Koehn, P. (2004, July). Statistical significance tests for machine translation evaluation. In Proceedings of the 2004 conference on empirical methods in natural language processing (pp. 388-395).

[3] Luu, K., Khashabi, D., Gururangan, S., Mandyam, K., \& Smith, N. A. (2022, July). Time Waits for No One! Analysis and Challenges of Temporal Misalignment. In Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (pp. 5944-5958).

[4] Grusky, M., Naaman, M., \& Artzi, Y. (2018). Newsroom: A dataset of 1.3 million summaries with diverse extractive strategies. arXiv preprint arXiv:1804.11283.

[5] Card, D., Boydstun, A., Gross, J. H., Resnik, P., \& Smith, N. A. (2015, July). The media frames corpus: Annotations of frames across issues. In Proceedings of the 53rd Annual Meeting of the Association for Computational Linguistics and the 7th International Joint Conference on Natural Language Processing (Volume 2: Short Papers) (pp. 438-444).

==> rebuttal/sections/review_4.tex <==
\newpage
\section{Review 4}
\label{sec:review-4}
Official Review of Submission1109 by Reviewer iqaY

\subsection*{Paper Topic And Main Contributions:}

The paper addresses the problem of temporal shift in text classification for time-series data with static pre-trained language models, where negatively impacts their performance over time. To address this issue, the authors propose two adaptation strategies: i) finetuning small language models with pseudo-labeled data (Online Buffered Self-Training), and ii) in-context learning with pseudo-labeled examples (Online Update of In-Context Examples). The authors conduct experiments on two datasets from public health (Covid19 vaccination stance detection dataset collected by the authors) and finance domains with evolving domain shifts on inputs and outputs, and demonstrate the effectiveness of their methods compared to unadapted baselines.



\subsection*{Reasons To Accept:}

The paper addresses an important topic in the literature, namely text classification in the presence of domain shift. The authors propose novel online and offline approaches that leverage a dynamic buffer of examples used for fine tuning or in-context learning domain adaptation.

Good selection of baselines to compare with; Insightful analysis demonstrating the importance of intermediate domains and the impact of errors on pseudo-labeling

The authors introduce a new evolving context dataset for Covid-19 vaccination, consisting of tweets which captures the public general stance towards vaccines


\subsection*{Reasons To Reject:}

\paragraph{1.} For the Online Update of In-Context Examples (OIE), the authors choose the example whose embedding is closest to the mean embedding of a class in terms of cosine similarity. However, the authors fail to acknowledge and discuss the sensitivity of In-Context Learning to the selection of training examples and issues such as recency bias, majority label bias, or the sensitivity of in-context learning to labels (issue particularly relevant as they rely on pseudo-labels)

\paragraph{2.} Lack of statistical significance test for the reported results

\paragraph{3.} In-Context Learning results (Figure3) do not seem very convincing; the source-only approach seems to be doing better than in-context learning for some domains

\paragraph{4.} No fine-grained analysis on why their method is working for some domains, while for other domains not so well

\paragraph{5.} More details for the hyper-paramter selection of their adaptation methods are needed

\paragraph{6.} The paper has limited novelty in terms of adaptation approaches, misses a significant body of literature on limitations of in-context learning, as well as methods in the literature that have explored the adaptation of language models to new text classification domains. Moreover, some of their findings are not rigorously explained and analyzed (see questions below).


\subsection*{Questions For The Authors:}

\paragraph{1.} It is interesting to see that for the medical dataset you chose CT-BERT, a pre-trained model on a large corpus of covid-19 tweets, while for the finance dataset you use a general purpose model when there are available open-source models pre-trained on financial data, for example https://huggingface.co/FinanceInc/finbert-pretrain . How do you motivate your choice of base models for adaptation?

\paragraph{2.} Lines 425 - 428: How do you explain the larger boost in performance for ChatGPT as opposed to the lack of improvement for FLAN-T5-XXL?

\subsection*{Missing References:} 

I recommend authors to check the literature on in-context learning and sensitivity to the selection of examples:

Zhao, Zihao, Eric Wallace, Shi Feng, Dan Klein, and Sameer Singh. "Calibrate before use: Improving few-shot performance of language models." In International Conference on Machine Learning, pp. 12697-12706. PMLR, 2021.

Lu, Yao, Max Bartolo, Alastair Moore, Sebastian Riedel, and Pontus Stenetorp. "Fantastically Ordered Prompts and Where to Find Them: Overcoming Few-Shot Prompt Order Sensitivity." In Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers), pp. 8086-8098. 2022.

Other papers that could be relevant: (focus on text classification) 

Suchin Gururangan, Ana Marasovic, Swabha Swayamdipta, Kyle Lo, Iz Beltagy	`	, Doug Downey, and Noah A Smith. ´ Don’t stop pretraining: Adapt language models to domains and tasks. In Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics, pp. 8342–8360, 2020.

(importance of intermediate datasets for adaptation) 

Garbacea, Cristina, and Qiaozhu Mei. "Adapting Pre-trained Language Models to Low-Resource Text Simplification: The Path Matters." In Conference on Lifelong Learning Agents, pp. 1103-1119. PMLR, 2022.

\subsection*{Ratings}

Soundness: 2: Borderline: Some of the main claims/arguments are not sufficiently supported, there are major technical/methodological problems
Excitement: 3: Ambivalent: It has merits (e.g., it reports state-of-the-art results, the idea is nice), but there are key weaknesses (e.g., it describes incremental work), and it can significantly benefit from another round of revision. However, I won't object to accepting it if my co-reviewers champion it.
Reproducibility: 3: Could reproduce the results with some difficulty. The settings of parameters are underspecified or subjectively determined; the training/evaluation data are not widely available.
Ethical Concerns: No
Reviewer Confidence: 5: Positive that my evaluation is correct. I read the paper very carefully and I am very familiar with related work.

\section*{\sn{Response to Review 4}}

\paragraph{Q1.} \textit{"Lines 425 - 428: How do you explain the larger boost in performance for ChatGPT as opposed to the lack of improvement for FLAN-T5-XXL?"}

Thank you for your valuable question! We believe that this may be due to the scaling effect since FLAN-T5-XXL is supposed to be a smaller model.  We would like to kindly refer you to our response to Reviewer lrUf's Q2. We expand the scope of LLMs and also conduct statistical significance test, and show that the benefit of OIE holds true for larger LLMs.

\paragraph{Q2.} \textit{"It is interesting to see that for the medical dataset you chose CT-BERT, a pre-trained model on a large corpus of covid-19 tweets, while for the finance dataset you use a general-purpose model when there are available open-source models pre-trained on financial data, for example https://huggingface.co/FinanceInc/finbert-pretrain. How do you motivate your choice of base models for adaptation?"}

Thank you for pointing us to FinBERT. We were not aware of FinBERT at the time of our initial submission. We rerun the experiment using FinBERT on WTWT comparing online buffered self-training (OBS) and online cumulative self-training (OCS) to the unadapted Src-Only baseline. For completeness, we also run the experiment with the generic BERT model (\textit{bert-uncased-large}) on COVID.

\input{rebuttal/tables/domain_specific_bert}

Interestingly, as shown in the table above, \textit{FinBERT} does not offer an improvement in model performance compared to the generic BERT. We suspect the reason is that the pretraining corpus of FinBERT (corporate reports, earning call transcripts etc.) has a distinct language style compared to tweets in WTWT. Nonetheless, the trend where OS>OCS>OBS>Src-Only in terms of the model performance holds true for \textit{FinBERT} on WTWT as well. On the other hand, CT-BERT does show a better overall performance compared to the generic BERT. Critically, regardless of which backbone model we choose, the benefit of OCS and OBS holds. 

\paragraph{Q3.} \textit{"The authors fail to acknowledge and discuss the sensitivity of In-Context Learning to the selection of training examples and issues such as recency bias, majority label bias, or the sensitivity of in-context learning to labels (issue particularly relevant as they rely on pseudo-labels)"}

Thank you for the question. We believe we have accounted for the biases you mentioned, but we did not state them clearly in the manuscript.

Regarding the majority label bias in our proposed online update of in-context examples (OIE), because each class has an equal number (exactly 1 example per class) of in-context examples in a prompt (line 4 to line 7 in Algorithm 2), no class has a higher count than other classes.

To address potential recency bias, we have randomly shuffled the in-context examples when we construct the prompt. That is, in Equation 3, the order of the in-context examples $\Ccal$ is randomly permuted across different queries. Therefore, within the in-context examples in the prompt, each class's label has an equal distance to the query tweet on average. Therefore, systematic recency bias should have been mitigated.

To evaluate the sensitivity to labels, we would like to kindly refer you to Table 4 in the paper, where we test the impact of inaccuracies in pseudo-labels. Indeed, because our methods rely on pseudolabels, the labeling error poses a potential threat to the performance of both OBS and OIE. When all the errors are manually corrected, the performance can be further improved. Nonetheless, even in the presence of labeling errors, OIE still outperforms the unadapted Src-Only baselines.

One may argue that OIE would not work for difficult tasks where the accuracy is low. To further test the efficacy of OIE in the presence of labeling errors, we additionally include two more challenging datasets from different areas. Please see the response to Q2 from Reviewer 24y4 for the results on the additional datasets. In short, the results echo the discoveries in our main paper, where OIE still outperforms the Src-Only baseline. Therefore, we believe that our proposed methods work for more challenging datasets as well, even when the base model performance is low.

\input{rebuttal/tables/oie_other_datasets}


\paragraph{Q4.} \textit{"Lack of statistical significance test for the reported results"}

Thank you for the suggestions. We have added the statistical test on OIE versus Src-Only (presented in the response to your question 1; we would also like to kindly refer you to our to Reviewer lrUf'Q2). 

In addition, we also conduct statistical tests on the differences between OS, OCS, OBS, and Src-Only. Similarly, for the statistical test on the results of OS, OCS, OBS, and Src-Only, we resample from the test set 1000 times, and derive the 95\% confidence interval of the difference between the following three model pairs: 1) OBS versus Src-Only, 2) OCS versus OBS, 3) OS versus OCS. For each bootstrapped sample, we compute the difference score $\Delta F_\text{avg}$ between two models in a pair. For example, for the comparison between OBS and Src-Only, $\Delta F_\text{avg}=(F_\text{avg} \text{of OBS}) - (F_\text{avg} \text{of Src-Only})$.

\input{rebuttal/tables/obs_bootstrap}

The result supports the claim that OS > OCS > OBS > Src-Only in terms of model performance.

\paragraph{Q5.} \textit{"In-Context Learning results (Figure 3) do not seem very convincing; the source-only approach seems to be doing better than in-context learning for some domains."}

Thank you for pointing this out. To test the robustness of our proposed online update of in-context examples (OIE), we expand the scope of LLMs (presented in our response to your Q1; we would also like to kindly refer you to our response to Reviewer 1rUf's Q2) and show that it generalizes to other LLMs as well. We also show that, \textit{averaged across all target domains}, OIE outperforms Src-Only for larger LLMs with statistical tests. In addition, we show that OIE works for more challenging datasets as well, even when the base model performance is low (presented in the response to your Q3; we also kindly refer you to the response to Q2 from Reviewer 24y4). 


\paragraph{Q6.}\textit{No fine-grained analysis on why their method is working for some domains, while for other domains not so well.}

Indeed, both OBS and OIE work better in some domains but not in others (Figure 2, 3, 5, 6 in the paper). We speculate that one possible factor is the distance between the source domain and the given target domain. As shown in the aforementioned Figures, the benefits of OBS and OIE become obvious when the distance between the source domain and the target domain arises. To formally test this hypothesis, we first derive the relative improvement in $F_{t}$ at each time step in the target domains. The relative improvement $\Delta F_{t}$ is defined as the improvement beyond the Src-only baseline in terms of macro-F1 score, divided by the Src-only baseline's macro-F1 score. For for OBS, $\Delta F_{OIE,t}=(\text{OBS's} F_{t}-\text{Src-Only's} F_{t}) / (\text{Src-Only's} F_{t})$ Likewise, for OIE, $\Delta F_{t, OIE}=(\text{OIE's} F_{t}-\text{Src-Only's} F_{t}) / (\text{Src-Only's} F_{t})$. 

We then compute the Pearson's correlation coefficient ($r$) between $\Delta F_{t}$ and the MMD distance $d_{t}$ between each target domain and the source domain. The Pearson's $r$ thus indicates how strongly the improvement of using buffer-based methods correlates with the degree of domain shift. The results are presented below. As shown in the table, the improvement of using OBS and OIE is associated with the degree of domain shift from the source domain.

\input{rebuttal/tables/spearman_rho}

\paragraph{Q7.} \textit{"More details for the hyper-parameter selection of their adaptation methods are needed"}

Thank you for offering us the chance to elaborate. For the hyperparameters for fine-tuning based methods (Src-only, OBS, OCS,OS), we have performed a grid search using Weights \& Biases. We explore the following hyperparameters: batch size (16, 32), learning rate ($2\times10^{-6},2\times10^{-5},2\times10^{-4},2\times10^{-3}$), a dropout rate of the attention layers (0.1, 0.3, 0.5), a dropout rate of the final linear layer (0, 0.1, 0.3). The grid search is performed based on the performance of the Src-only baseline model, while retaining the configuration with the highest $F_\text{avg}$ in the validation set.

Aside from the aforementioned hyperparameters, we further test the methods' sensitivity to the sliding window size. We would like to kindly refer you to our response to reviewer 4Jm5's Q4. The overall trend of results remains the same with different window sizes.

\paragraph{Q8.} \textit{"The paper misses methods in the literature that have explored the adaptation of language models to new text classification domains."}

Thanks for the helpful suggestion. We provide additional results on two more baseline methods: DANN and DAPT. We would like to kindly refer you to our response to Q1 from Reviewer 24y4. In short, while DANN and DAPT outperforms the Src-Only baseline, they still underperform OBS.

\subsection*{References}

[1] Koehn, P. (2004, July). Statistical significance tests for machine translation evaluation. In Proceedings of the 2004 conference on empirical methods in natural language processing (pp. 388-395).

[2] Ganin, Y., Ustinova, E., Ajakan, H., Germain, P., Larochelle, H., Laviolette, F., ... \& Lempitsky, V. (2016). Domain-adversarial training of neural networks. The journal of machine learning research, 17(1), 2096-2030.

[3] Tzeng, E., Hoffman, J., Saenko, K., \& Darrell, T. (2017). Adversarial discriminative domain adaptation. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 7167-7176).

[4] Gururangan, S., Marasović, A., Swayamdipta, S., Lo, K., Beltagy, I., Downey, D., \& Smith, N. A. (2020, July). Don’t Stop Pretraining: Adapt Language Models to Domains and Tasks. In Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics (pp. 8342-8360).

[5] Luu, K., Khashabi, D., Gururangan, S., Mandyam, K., \& Smith, N. A. (2022, July). Time Waits for No One! Analysis and Challenges of Temporal Misalignment. In Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (pp. 5944-5958).


==> rebuttal/tables/domain_specific_bert.tex <==
\begin{table}[H]
  \centering  
  \small
  \begin{tabular}{lllll}
    \toprule
    Method & \multicolumn{2}{c}{Generic BERT} & \multicolumn{2}{c}{Specific BERT} \\ 
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    & COVID & WTWT & COVID & WTWT \\
    \midrule
    \tunesource & 0.552 & 0.618 & 0.720 & 0.601 \\
    \onlinebuf & 0.589 & 0.697 & 0.778 & 0.671 \\
    \onlinecum & 0.629 & 0.739 & 0.800 & 0.708 \\
    \offline & 0.683 & 0.789 & 0.832 & 0.763 \\
    \toprule
    \tunetrue & 0.687 & 0.785 & 0.835 & 0.767 \\
    \bottomrule
  \end{tabular}
  \caption{$F_\text{avg}$ (the macro-average F1 score averaged across all target domains) for our proposed methods across generic (\textit{bert-uncased-large}) and domain-specific BERT (\textit{CT-BERT} for COVID and \textit{FinBERT} for WTWT).}
  \vspace{-5mm}
\end{table}


==> rebuttal/tables/more_llms.tex <==
\begin{table}[H]
  \centering
  \small
   \resizebox{\linewidth}{!}{
  \begin{tabular}{llll}
    \toprule
    \multirow{2}{*}{Model}  & In-context & \multicolumn{2}{c}{Dataset} \\ 
    \cmidrule{3-4}
    & Examples & COVID & WTWT \\
    \midrule
    \multirow{3}{*}{ChatGPT} & \promptzero & 0.746 & 0.590 \\
    & \promptsource & 0.780 & 0.632 \\
    & \onlineexp & 0.791 & 0.645 \\
    \cmidrule{1-4}    
    \multirow{3}{*}{\textbf{davinci-003 (175B)}} & \promptzero & 0.695 & 0.575 \\
    & \promptsource & 0.744 & 0.612 \\
    & \onlineexp & 0.752 & 0.620 \\
    \cmidrule{2-4}    
    \multirow{3}{*}{\textbf{curie-001 (13B)}} & \promptzero & 0.275 & 0.435 \\
    & \promptsource & 0.521 & 0.481 \\    
    & \onlineexp & 0.526 & 0.488 \\   
    \cmidrule{2-4}   
    \multirow{3}{*}{\textbf{babbage-001 (3B)}} & \promptzero & 0.276 & 0.415 \\
    & \promptsource & 0.409 & 0.445 \\
    & \onlineexp & 0.411 & 0.448 \\            
    \cmidrule{1-4}
    \multirow{3}{*}{\textbf{FLAN-UL2 (20B)}} & \promptzero & 0.788 & 0.585 \\
    & \promptsource & 0.790 & 0.591 \\
    & \onlineexp & 0.794 & 0.596 \\        
    \cmidrule{2-4}
    \multirow{3}{*}{FLAN-T5-XXL (11B)} & \promptzero & 0.779 & 0.560 \\
    & \promptsource & 0.784 & 0.562 \\
    & \onlineexp & 0.788 & 0.563 \\    
    \cmidrule{2-4}
    \multirow{3}{*}{\textbf{FLAN-XL (3B)}} & \promptzero & 0.723 & 0.529 \\
    & \promptsource & 0.730 & 0.531 \\
    & \onlineexp & 0.732 & 0.531 \\            
    \toprule
     BERT (\tunetrue)  & - & 0.835 & 0.785 \\
    \bottomrule
  \end{tabular} 
  }
  \caption{Performance metrics for prompting different LLMs with different number of parameters on the two datasets. The metric presents $F_\text{avg}$, the macro-average F1 score averaged across all target domains. The supervised tuning-based method baseline is also included as a reference. Texts in bold highlight the additional results we add to the original submission.}
\end{table}


==> rebuttal/tables/obs_bootstrap.tex <==
\begin{table}[H]
  \centering
  \small
   \resizebox{\linewidth}{!}{
  \begin{tabular}{lll}
    \toprule
    \multirow{2}{*}{Constast}  & \multicolumn{2}{c}{$\Delta F_\text{avg}$ (OIE$-$Src-Only)} \\ 
    \cmidrule{2-3}
    & COVID & WTWT \\
    \toprule    
    OBS$-$Src-only & 0.056 [0.050, 0.061] & 0.077 [0.070, 0.085] \\
    OCS$-$OBS & 0.021 [0.015, 0.025] & 0.042 [0.036, 0.050] \\
    OS$-$OCS & 0.031 [0.025, 0.038] & 0.051 [0.042, 0.059] \\    
    \bottomrule
  \end{tabular} 
  }
  \caption{Bootstrapping results through 1000 paired bootstrap resampling. Metrics present the median of difference in $F_\text{avg}$ between two models in a contrast pair. For example, for the constras between OIE and the Src-only baseline, $\Delta F_\text{avg}$ is the $F_\text{avg}$ of OBS minus the $F_\text{avg}$ of Src-only. The 95\% bootstrap confidence interval is shown in brackets. $F_\text{avg}$ is the macro-average F1 score averaged across all target domains.}
\end{table}



==> rebuttal/tables/obs_other_datasets.tex <==
\begin{table}[H]
  \centering  
  \small
  \begin{tabular}{lll}
    \toprule
    Method & \multicolumn{2}{c}{Dataset} \\ 
    \cmidrule{2-3}
    & SCIERC & PUBCLS \\
    \midrule
    \tunesource & 0.485 & 0.406 \\
    \onlinebuf & 0.520 & 0.469 \\
    \onlinecum & 0.684 & 0.492 \\
    \offline & 0.814 & 0.626 \\
    \toprule
    \tunetrue & 0.822 & 0.651 \\
    \bottomrule
  \end{tabular}
  \caption{Performance metrics for fine-tuning based methods on the two additional datasets. $F_\text{avg}$ (the macro-average F1 score averaged across all target domains) for our proposed methods in other datasets}
  \vspace{-5mm}
\end{table}


==> rebuttal/tables/oie_bootstrap.tex <==
\begin{table}[H]
  \centering
  \small
   \resizebox{\linewidth}{!}{
  \begin{tabular}{lll}
    \toprule
    \multirow{2}{*}{Model}  & \multicolumn{2}{c}{$\Delta F_\text{avg}$ (OIE$-$Src-Only)} \\ 
    \cmidrule{2-3}
    & COVID & WTWT \\
    \toprule    
    ChatGPT & 0.011 [0.006, 0.017] & 0.013 [0.008, 0.017] \\
    davinci-003 (175B) & 0.008 [0.003, 0.012] & 0.009 [0.002, 0.015] \\
    curie-001 (13B) & 0.005 [-0.001, 0.009] & 0.007 [0.001, 0.014] \\
    babbage-001 (3B) & 0.002 [-0.002, 0.007] & 0.003 [-0.004, 0.010] \\
    FLAN-T5-UL2 (20B) & 0.005 [0.001, 0.010] & 0.003 [-0.004, 0.009] \\
    FLAN-T5-XXL (11B) & 0.004 [0.0008, 0.010] & 0.001 [-0.003, 0.006] \\
    FLAN-T5-XL (3B) & 0.001 [-0.005, 0.006] & 0.000 [-0.004, 0.005] \\
    \bottomrule
  \end{tabular} 
  }
  \caption{Bootstrapping results through 1000 paired bootstrap resampling. Metrics present the median of difference in $F_\text{avg}$ between OIE and the Src-only baseline ($F_\text{avg}$ of OIE minus $F_\text{avg}$ of Src-only). The 95\% bootstrap confidence interval is shown in brackets. $F_\text{avg}$ is the macro-average F1 score averaged across all target domains.}
\end{table}



==> rebuttal/tables/oie_other_datasets.tex <==
\begin{table}[H]
  \centering
  \small
   \resizebox{\linewidth}{!}{
  \begin{tabular}{llll}
    \toprule
    \multirow{2}{*}{Model}  & In-context & \multicolumn{2}{c}{Dataset} \\ 
    \cmidrule{3-4}
    & Examples & SCIERC & PUBCLS \\
    \midrule
    \multirow{3}{*}{ChatGPT} & \promptzero & 0.272 & 0.538 \\
    & \promptsource & 0.320 & 0.568 \\
    & \onlineexp & 0.352 & 0.591 \\
    \bottomrule
  \end{tabular} 
  }
  \caption{Performance metrics for prompting two LLMs on the two additional datasets. The metric presents $F_\text{avg}$, the macro-average F1 score averaged across all target domains.}
\end{table}


==> rebuttal/tables/other_adapted_methods.tex <==
\begin{table}[H]
  \centering  
  \small
  \begin{tabular}{lll}
    \toprule
    Method & \multicolumn{2}{c}{Dataset} \\ 
    \cmidrule{2-3}
    & COVID & WTWT \\
    \midrule
    \tunesource & 0.720 & 0.618 \\
    \onlinebuf & 0.778 & 0.697 \\
    \onlinecum & 0.800 & 0.739 \\
    \offline & 0.832 & 0.789 \\
    \midrule
    \textbf{DANN} & 0.751 & 0.647 \\
    \textbf{DAPT} & 0.727 & 0.679 \\
    \toprule
    \tunetrue & 0.835 & 0.785 \\
    \bottomrule
  \end{tabular}
  \caption{$F_\text{avg}$ (the macro-average F1 score averaged across all target domains) for our proposed methods versus other adaptation methods (DANN, DAPT). Texts in bold highlight the additional results we add to the original submission.}
  \vspace{-5mm}
\end{table}


==> rebuttal/tables/spearman_rho.tex <==
\begin{table}[H]
  \centering  
  \small
  \begin{tabular}{lll}
    \toprule
    Method & \multicolumn{2}{c}{Dataset} \\ 
    \cmidrule{2-3}
    & COVID & WTWT \\
    \midrule
    OBS & 0.577 & 0.643 \\
    OIE & 0.298 & 0.383 \\
    \bottomrule
  \end{tabular}
  \caption{The Pearson's $r$ between $\Delta F_{t}$ and $d_{t}$ for both datasets.}
  \vspace{-5mm}
\end{table}


==> rebuttal/tables/varying_window_size.tex <==
\begin{table}[H]
  \centering  
  \small
  \begin{tabular}{llll}
    \toprule
    Window Size & Method & \multicolumn{2}{c}{Dataset} \\ 
    \cmidrule{3-4}
    & & COVID & WTWT \\
    \midrule
    - & \tunesource & 0.720 & 0.618 \\   
    \midrule         
    1 month & \onlinebuf & 0.778 & 0.712 \\
     & \onlinecum & 0.800 & 0.745 \\
    \cmidrule{2-4}     
    2 month & \onlinebuf & 0.767 & 0.697 \\
     & \onlinecum & 0.780 & 0.739 \\
    \cmidrule{2-4}          
    3 month & \onlinebuf & 0.752 & 0.652 \\
     & \onlinecum & 0.777 & 0.709 \\
    \midrule     
   - & \offline & 0.832 & 0.789 \\
    \toprule
   - & \tunetrue & 0.835 & 0.785 \\
    \bottomrule
  \end{tabular}
  \caption{$F_\text{avg}$ (the macro-average F1 score averaged across all target domains) for different sliding window sizes}
  \vspace{-5mm}
\end{table}


==> tables/ablation_intermediate.tex <==
\begin{table}[tbp!]
  \centering  
  \small
  \resizebox{\linewidth}{!}{  
      \begin{tabular}{llllll}
        \toprule
        Approach & Method & \multicolumn{4}{c}{Dataset} \\ 
        \cmidrule{3-6}
        & & COVID & WTWT & SCIERC & PUBCLS\\
        \midrule
        \multirow{2}{*}{Tuning} & \tunesource & 0.491 & 0.640 & 0.480 & 0.280 \\
         & \onlinebuf & 0.686 & 0.763 & 0.583 &0.494 \\
         & \tuneablate & 0.502 & 0.652 & & \\     
        \midrule
        \multirow{2}{*}{Prompting} & \promptsource & 0.766 & 0.581 & & \\
         & \onlineexp & 0.797 & 0.585  & & \\
         & \promptablate & 0.771 & 0.572  & & \\
        % \toprule
        % \tunetrue & - & 0.857 & 0.817 \\
        \bottomrule
      \end{tabular}
    }  
  \caption{Ablation study evaluating the importance of intermediate domains. The method \tuneablate stands for the ablated condition where the intermediate domains are removed. The performance metric is $F_{\text{macro},T}$.}
  \label{tab:ablataion_inter}
\end{table}



==> tables/ablation_pseudolabeling_error.tex <==
\begin{table}[htbp!]
  \centering  
  \small
  \begin{tabular}{llll}
    \toprule
    Method & Perturbation & \multicolumn{2}{c}{Dataset} \\ 
    \cmidrule{3-4}
    & & COVID & WTWT \\
    \midrule
    \multirow{4}{*}{\onlinebuf} & Corrected & 0.794 & 0.721 \\
     & 0\% & 0.778 & 0.697 \\
     & 10\% & 0.730 & 0.649 \\    
     & 50\% & 0.523 & 0.498 \\
     % & Corrected &
    \midrule
    \multirow{4}{*}{\onlineexp} & Corrected & 0.796 & 0.646 \\
     & 0\% & 0.791 & 0.645 \\    
     & 10\% & 0.761 & 0.629 \\    
     & 50\% & 0.697 & 0.481 \\
    % \toprule
    % \tunetrue & - & 0.857 & 0.817 \\
    \bottomrule
  \end{tabular}
  \caption{Impact of pseudo-labeling errors on model performance. The performance metric ($F_\text{avg}$) of both \onlinebuf and \onlineexp methods is evaluated with varying levels of induced pseudo-labeling errors (from 0\% to 50\%). The "Corrected" row serves as an upper performance bound with access to error-free pseudo-labels.}
  \label{tab:ablataion_pseudo_error}
\end{table}



==> tables/main_result_prompting.tex <==
\begin{table}[tbp!]
  \centering
  \small
  \resizebox{\linewidth}{!}{
  \begin{tabular}{llllll}
    \toprule
    \multirow{2}{*}{Model}  & In-context & \multicolumn{4}{c}{Dataset} \\ 
    \cmidrule{3-6}
    & Examples & COVID & WTWT & SCIERC & PUBCLS \\
    \midrule
    \multirow{3}{*}{ChatGPT} & \promptzero & 0.746 & 0.590 & 0.272 & 0.538 \\
    & \promptsource & 0.780 & 0.632 & \textbf{0.352} & 0.568 \\
    & \onlineexp & \textbf{0.791} & \textbf{0.645} & 0.320 & \textbf{0.591} \\
    \cmidrule{1-6}    
    \multirow{3}{*}{davinci-003 (175B)} & \promptzero & 0.695 & 0.575 & 0.245 & 0.588 \\
    & \promptsource & 0.744 & 0.612 & \textbf{0.331} & 0.587 \\
    & \onlineexp & \textbf{0.752} & \textbf{0.620} & 0.303 & \textbf{0.623} \\
    \cmidrule{1-6}    
    \multirow{3}{*}{curie-001 (13B)} & \promptzero & 0.275 & 0.435 & 0.263 & 0.471 \\
    & \promptsource & 0.521 & 0.481 & \textbf{0.291} & 0.522 \\    
    & \onlineexp & \textbf{0.526} & \textbf{0.488} & 0.270 & \textbf{0.532} \\
    \cmidrule{1-6}   
    \multirow{3}{*}{babbage-001 (3B)} & \promptzero & 0.276 & 0.415 & 0.212 & 0.462 \\
    & \promptsource & 0.409 & 0.445 & \textbf{0.281} & 0.491 \\
    & \onlineexp & \textbf{0.411} & \textbf{0.448} & 0.257 & \textbf{0.493} \\            
    \cmidrule{1-6}
    \multirow{3}{*}{FLAN-UL2 (20B)} & \promptzero & 0.788 & 0.585 & 0.455 & 0.520 \\
    & \promptsource & 0.790 & 0.591 & 0.458 & 0.569 \\
    & \onlineexp & \textbf{0.794} & \textbf{0.596} & \textbf{0.467} & \textbf{0.577} \\
    \cmidrule{1-6}
    \multirow{3}{*}{FLAN-T5-XXL (11B)} & \promptzero & 0.779 & 0.560 & 0.359 & 0.569 \\
    & \promptsource & 0.784 & 0.562 & 0.463 & 0.621 \\
    & \onlineexp & \textbf{0.788} & \textbf{0.563} & \textbf{0.465} & \textbf{0.632} \\
    \cmidrule{1-6}
    \multirow{3}{*}{FLAN-XL (3B)} & \promptzero & 0.723 & 0.529 & 0.290 & 0.520 \\
    & \promptsource & 0.730 & \textbf{0.531} & \textbf{0.312} & 0.533 \\
    & \onlineexp & \textbf{0.732} & \textbf{0.531} & 0.287 & \textbf{0.536} \\
    \toprule
    BERT (\tunetrue)  & - & 0.835 & 0.785 & 0.822 & 0.651 \\
    \bottomrule
  \end{tabular} 
  }
  \caption{Performance metrics for prompting two LLMs on all datasets. The metric presents $F_\text{avg}$, the macro-average F1 score averaged across all target domains. The supervised tuning-based method baseline is also included as a reference.}
  \label{tab:performance_metrics_prompting}
\end{table}


==> tables/main_result_tuning_bert.tex <==
\begin{table}[tbp!]
  \centering  
  % \small
   \resizebox{\linewidth}{!}{  
  \begin{tabular}{llllll}
    \toprule
    Methods & Variants & \multicolumn{4}{c}{Dataset} \\ 
    \cmidrule{3-6}
    & & COVID & WTWT & SCIERC & PUBCLS \\
    \midrule
    Baseline & \tunesource & 0.509 & 0.618 & 0.485 & 0.406 \\
    \midrule       
    Self-training & \offline & 0.460 (-28) & 0.633 (9) & 0.593 (32) & 0.363 (-18)\\    
     & \onlinebuf  & 0.569 (34) & 0.697 (47) & 0.520 (10) & 0.469 (26) \\
     & \onlinecum  & \textbf{0.611 (57)} & \textbf{0.739 (72)} & \textbf{0.684 (59)} & \textbf{0.492 (35)} \\
    % \midrule       
    DANN & - & 0.519 (6) & 0.647 (17) & 0.511 (8) & 0.440 (14)\\
    DAPT & - & 0.524 (8) & 0.664 (28) & 0.503 (5) & 0.458 (21)\\
    \midrule    
    \tunetrue & - & 0.687 & 0.785 & 0.822 & 0.651 \\    
    \bottomrule
  \end{tabular}
  }
  \caption{Performance metrics across methods for the BERT-large model on all datasets. Each entry shows $F_\text{avg}$, as well as $\Delta_{\text{avg,norm}}$ for each adaptive method, shown in percentage in the parentheses (\%).}
  \label{tab:performance_metrics_tuning_bert}
  \vspace{-3mm}
\end{table}


==> tables/main_result_tuning_flant5.tex <==
\begin{table}[tbp!]
  \centering  
  \small
   \resizebox{\linewidth}{!}{  
      \begin{tabular}{llll}
        \toprule
        Methods & Variants & \multicolumn{2}{c}{Dataset} \\ % change moulti column from {4}{c} to {3}{c}
        \cmidrule{3-4} % change from {3-6} to {3-5}
        & & COVID & SCIERC  \\
        \midrule    
        \promptzero & - & 0.772  &  0.348 \\
        \midrule
        Baseline & \tunesource & 0.795  &  0.809 \\
        \midrule       
        Self-training & \offline & 0.816 (46)  &  0.820 (22) \\    
         & \onlinebuf  & 0.812 (37) &  0.822 (39)\\    
         & \onlinecum  & \textbf{0.821 (57)}  & \textbf{0.842 (100)} \\
        % \midrule       
        DAPT & - & 0.731 (<0)  & 0.503 (<0)\\   %WTWT was 0.664
        \midrule    
        \tunetrue & - & 0.841 & 0.842 \\    % WTWT was ? before
        \bottomrule
      \end{tabular}
  }
  \caption{Performance metrics across methods for the FLAN-T5-XXL model on all datasets. Each entry shows $F_\text{avg}$, as well as $\Delta_{\text{avg,norm}}$ for each adaptive method, shown in percentage in the parentheses (\%).}
  \label{tab:performance_metrics_tuning_flant5}
  \vspace{-5mm}
\end{table}


% \begin{table}[tbp!]
%   \centering  
%   \small
%    \resizebox{\linewidth}{!}{  
%       \begin{tabular}{lllll}
%         \toprule
%         Methods & Variants & \multicolumn{3}{c}{Dataset} \\ % change moulti column from {4}{c} to {3}{c}
%         \cmidrule{3-5} % change from {3-6} to {3-5}
%         & & COVID & SCIERC & PUBCLS \\
%         \midrule    
%         \promptzero & - & 0.772  &  0.348 & -\\
%         \midrule
%         Baseline & \tunesource & 0.795  &  0.809 & -\\
%         \midrule       
%         Self-training & \offline & 0.816  &  0.820 & -\\    
%          & \onlinebuf  & 0.812  &  0.822 & - \\    
%          & \onlinecum  & \textbf{0.821}  & \textbf{0.842} & -\\
%         % \midrule       
%         DAPT & - & 0.731  & 0.503 & 0.458  \\   %WTWT was 0.664
%         \midrule    
%         \tunetrue & - & 0.841 & 0.842 & - \\    % WTWT was ? before
%         \bottomrule
%       \end{tabular}
%   }
%   \caption{Performance metrics ($F_\text{avg}$) across methods for the FLAN-T5-XXL model on all datasets except WTWT. \sn{Should also mention the Zero baseline}}
%   \label{tab:performance_metrics_tuning}
%   \vspace{-5mm}
% \end{table}


